Delay-Augmented Stacked Intelligent Surfaces: Potential, Challenges, and Opportunities

Stacked intelligent surfaces (SIS)s have been proposed recently as an enabling technology for Holographic Multiple Input Multiple Output (HMIMO) and Ultra-massive MIMO (umMIMO) technologies. Their utility can extend beyond spatial wave-domain processing of signals if they are enhanced with strategically-tuned symbol-duration level delays to enable temporal processing as well. In this work, we introduce the idea of a delay-augmented SIS (DA-SIS). We shed light on the feasibility of realizing delay units in an SIS. Then, we discuss the relevance of the proposed DA-SIS and present a use case that illustrates its potential, wherein the DA-SIS serves as an analog equalizer that aids in eliminating multi-path-induced inter-symbol-interference (ISI). We show how the number of elements affect the equalization process using the bit error rate (BER) as a metric, and demonstrate the potential of the DA-SIS in equalization via comparing with digital equalizers as a benchmark. Finally, we present opportunities and future research directions that can be undertaken to bring this idea to fruition.

==> Images/berfinals.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=40,
xmax=65,
xlabel style={at={(axis cs: 51,0.00001)},font=\color{white!15!black}},
xlabel={SNR (dB)},
xtick={40,45,50,55,60,65},
xticklabels={40,45,50,55,60,65},
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
ylabel style={at={(axis cs: 40,0.003)},font=\color{white!15!black}},
ylabel={BER},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(axis cs: 41,0.000015)}, anchor = south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, line width=1.0pt]
  table[row sep=crcr]{%
40	0.453692031872511\\
41	0.442021314741037\\
42	0.427609163346615\\
43	0.410025298804782\\
44	0.388546613545818\\
45	0.363653784860557\\
46	0.3353093625498\\
47	0.305018127490039\\
48	0.274669322709162\\
49	0.247056175298805\\
50	0.223765139442232\\
51	0.206878884462152\\
52	0.197993027888447\\
53	0.197975498007969\\
54	0.205232270916335\\
55	0.217316533864543\\
56	0.22998266932271\\
57	0.240254980079682\\
58	0.246697609561753\\
59	0.249321314741034\\
60	0.249959760956175\\
61	0.249993824701195\\
62	0.249994621513944\\
63	0.249991633466136\\
64	0.250005976095618\\
65	0.250007768924303\\
66	0.249998207171315\\
67	0.250014143426295\\
68	0.249987450199203\\
69	0.250005976095618\\
70	0.250006175298805\\
};
\addlegendentry{No equalization}

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
40	0.4822746\\
41	0.477463200000001\\
42	0.472005600000001\\
43	0.4644408\\
44	0.4556856\\
45	0.444524\\
46	0.4297248\\
47	0.411981199999999\\
48	0.389320999999999\\
49	0.3622834\\
50	0.3287296\\
51	0.288950999999999\\
52	0.2408204\\
53	0.1884494\\
54	0.132698\\
55	0.0814099999999997\\
56	0.0395902\\
57	0.0136774\\
58	0.00278479999999999\\
59	0.0002282\\
60	5.2e-06\\
61	2e-07\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{IIR ZF}

\addplot [color=blue, dashed, line width=1.0pt]
  table[row sep=crcr]{%
40	0.4514978\\
41	0.4389626\\
42	0.4234866\\
43	0.403850399999999\\
44	0.3797702\\
45	0.349737800000001\\
46	0.3133644\\
47	0.270088799999999\\
48	0.2202108\\
49	0.1658902\\
50	0.1107552\\
51	0.0618250000000001\\
52	0.0263391999999999\\
53	0.0073252\\
54	0.0010778\\
55	5.6e-05\\
56	6.00000000000001e-07\\
57	0\\
58	0\\
59	0\\
60	0\\
61	0\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{IIR ZF (noiseless eq.)}

\addplot [color=red, line width=1.0pt]
  table[row sep=crcr]{%
40	0.471311000000001\\
41	0.464005800000001\\
42	0.454671400000001\\
43	0.443251600000001\\
44	0.4286938\\
45	0.411217399999999\\
46	0.388726799999999\\
47	0.361737200000001\\
48	0.3296648\\
49	0.29348\\
50	0.2524894\\
51	0.2103564\\
52	0.1700206\\
53	0.1346736\\
54	0.1055292\\
55	0.0826147999999995\\
56	0.0642768\\
57	0.0490199999999998\\
58	0.0356302\\
59	0.0229487999999999\\
60	0.0123068\\
61	0.0048274\\
62	0.0012342\\
63	0.0001384\\
64	6.40000000000001e-06\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{FIR ZF ($4$ taps)}

\addplot [color=red, dashed, line width=1.0pt]
  table[row sep=crcr]{%
40	0.479828800000001\\
41	0.474624600000001\\
42	0.468107400000001\\
43	0.459712600000001\\
44	0.4499856\\
45	0.4372832\\
46	0.4205712\\
47	0.400905399999999\\
48	0.3759166\\
49	0.346567400000001\\
50	0.3105244\\
51	0.269418399999999\\
52	0.2229352\\
53	0.175378\\
54	0.1291612\\
55	0.0897467999999995\\
56	0.0582684\\
57	0.0359769999999999\\
58	0.0204771999999999\\
59	0.00987819999999999\\
60	0.003479\\
61	0.000706200000000001\\
62	6.68000000000001e-05\\
63	2.2e-06\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{FIR ZF ($20$ taps)}

\addplot [color=black, line width=1.0pt, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
40	0.491825\\
41	0.4901088\\
42	0.486585000000001\\
43	0.4832594\\
44	0.479058000000001\\
45	0.474162200000001\\
46	0.467450800000001\\
47	0.459531200000001\\
48	0.448374\\
49	0.4352706\\
50	0.4185962\\
51	0.398053199999999\\
52	0.3720396\\
53	0.3418286\\
54	0.3046148\\
55	0.260496199999999\\
56	0.2113692\\
57	0.1594288\\
58	0.1089914\\
59	0.065633\\
60	0.0334298\\
61	0.0136762\\
62	0.0039088\\
63	0.000669800000000001\\
64	5.04e-05\\
65	1.4e-06\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{DA-SIS  $N=4$}

\addplot [color=black, line width=1.0pt, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
40	0.470783800000001\\
41	0.462918800000001\\
42	0.453325\\
43	0.4411392\\
44	0.4268202\\
45	0.407818599999999\\
46	0.384181999999999\\
47	0.355557400000001\\
48	0.32067\\
49	0.279003199999999\\
50	0.231350200000001\\
51	0.177765\\
52	0.1234182\\
53	0.0741735999999996\\
54	0.0358709999999999\\
55	0.0126906\\
56	0.0029588\\
57	0.0003668\\
58	1.48e-05\\
59	2e-07\\
60	0\\
61	0\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{DA-SIS $N=25$}

\addplot [color=black, line width=1.0pt, mark=square, mark options={solid, black}]
  table[row sep=crcr]{%
40	0.436751\\
41	0.420545\\
42	0.400522399999999\\
43	0.3755156\\
44	0.345023800000001\\
45	0.3080458\\
46	0.264255799999999\\
47	0.214792\\
48	0.1615248\\
49	0.10952\\
50	0.0639337999999999\\
51	0.0307856\\
52	0.0114492\\
53	0.0028814\\
54	0.0004148\\
55	2.4e-05\\
56	0\\
57	0\\
58	0\\
59	0\\
60	0\\
61	0\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
};
\addlegendentry{DA-SIS $N=81$}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
